Socially-Informed Timeline Generation for Complex Events

Existing timeline generation systems for complex events consider only information from traditional media, ignoring the rich social context provided by user-generated content that reveals representative public interests or insightful opinions. We instead aim to generate socially-informed timelines that contain both news article summaries and selected user comments. We present an optimization framework designed to balance topical cohesion between the article and comment summaries along with their informativeness and coverage of the event. Automatic evaluations on real-world datasets that cover four complex events show that our system produces more informative timelines than state-of-the-art systems. In human evaluation, the associated comment summaries are furthermore rated more insightful than editor's picks and comments ranked highly by users.

==> framework.tex <==
Our framework 

==> graphreg.tex <==
Before we describe our timeline generation framework, we first introduce a joint learning method based on \textit{graph regularization} that can learn the ranking functions for article sentences and social context simultaneously.

%Meanwhile, if we want to generate a coherent summary where the users can tell which event the comments refer to, we'd better do the selection at the same time. So it might be possible that we can learn two ordering functions simultaneously, one for the sentences in news articles and the other for the social context.

Suppose in the training data, we have a set of documents $\{d_{i}\}$. For each document, we have a set of sentences $\{s_{ij}\}$ and a set of comments $\{c_{ik}\}$. We know the human abstract for each document, so that we can compute a ROUGE score for each sentence. For comments we assign a comment value of $1.0$ if it is an editor-pick and $0.0$ otherwise.

%We also can construct a bipartite graph between the sentences and comments, the weight on the edge could be the textual similarity between the sentence and the comment (we can use other metrics as well, and I think I should think about this). 

Formally, our goal is to learn two rankers to give preference orderings on the sentences and comments for each article. We consider a simple linear regression model for predicting the importance of each sentence and insightfulness of each comment.


\subsection{Articles Sentence Importance}
For each sentence $x_{s}$ we have a corresponding feature vector $\mathbf{x_{s}}$ and a gold-standard score $y_{s}$. Gold-standard scores are computed against the human abstracts with ROUGE-2 scores. Sentences in the training set are denoted $\mathbf{X_{s}}$, with labels $\mathbf{Y_{s}}$. The importance of a sentence is scored as $f(x_{s})=\mathbf{x_{s}}\cdot \mathbf{w_{s}}$, where $\mathbf{w_{s}}$ is a weight vector to be estimated. For a standard linear regression classifier, we have the objective function below:

{\scriptsize
\begin{equation}
\begin{split}
F_{s, 1}(\mathbf{w_{s}})&=\alpha_{s}\cdot ||\mathbf{X_{s}} \mathbf{w_{s}}- \mathbf{Y_{s}}||_{2} + \beta_{s}\cdot ||\mathbf{X_{s}}||_{2}\\
%&=\alpha_{s}\cdot (\mathbf{w_{s}^{T}}\mathbf{X_{s}^{T}} -\mathbf{Y_{s}^{T}})(\mathbf{X_{s}} \mathbf{w_{s}}-\mathbf{Y_{s}}) + \beta_{s}\cdot ||\mathbf{X_{s}}||_{2}
\end{split}
\end{equation}
}

Because the first sentence in the article usually plays a very important role, we also consider minimizing pairwise loss between the first sentence and other sentences in the same article.

{\scriptsize
\begin{equation}
\begin{split}
&F_{s, 2}(\mathbf{w_{s}})=F_{s, 1}(\mathbf{w_{s}}) +\\
& \lambda_{position}\cdot \sum_{a}\sum_{i\neq 0, x_{i}\in a} ||(\mathbf{x_{a,0}}-\mathbf{x_{a,i}})\mathbf{w_{s}}- (l_{a,0}-l_{a,i})||_{2}\\
&=F_{s, 1}(w_{s}) +\lambda_{position}\cdot \mathbf{w_{s}^{T}}\mathbf{X_{s}^{T}}\mathbf{L_{position}}\mathbf{X_{s}}\mathbf{w_{s}}
\end{split}
\end{equation}
}

where $a$ is an article in the collection, and $L_{position}$ is graph Laplacian defined based on an adjacency matrix between the first sentence and other sentences. This regularizar encodes the information that the importance of the first sentence should be larger than the other sentences in the article.


\subsection{Social Context Importance}
For each comment $x_{c}$ we have a corresponding feature vector $\mathbf{x_{c}}$ and a gold-standard label $y_{c}$ indicating editor-pick comments. All the comments in the training set are denoted $\mathbf{X_{c}}$ with labels $\mathbf{Y_{c}}$. Notice that we use graph regularization in this framework, which means we can use semi-supervised learning and leverage the unlabeled data in the training phase. For example, in addition to 2,226 articles with comments labeled as editor-picks or not, there are 1,537 articles containing comments without any editor-pick labels. We use both sets for training.

Again as a standard linear regression classifier, we have an objective function:

{\scriptsize
\begin{equation}
\begin{split}
F_{c, 1}(\mathbf{w_{c}})&=\alpha_{c}\cdot ||\mathbf{X_{c}} \mathbf{w_{c}}, \mathbf{Y_{c}}||_{2} + \beta_{c}\cdot ||\mathbf{X_{c}}||_{2}\\
%&=\alpha_{c}\cdot (\mathbf{w_{c}^{T}}\mathbf{X_{c}^{T}} -\mathbf{Y_{c}^{T}})(\mathbf{X_{c}} \mathbf{w_{c}}-\mathbf{Y_{c}}) + \beta_{c}\cdot ||\mathbf{X_{c}}||_{2}
\end{split}
\end{equation}
}

We will consider two types of regularizing constraints: one for the pairwise ranking, and the other for the author information. The pairwise rankings has been used in rank SVM as hard constraints, but in our case they are soft constraints. %why?

{\scriptsize
\begin{equation}
\begin{split}
%F_{c, 2}(\mathbf{w_{c}})&=F_{c, 1}(\mathbf{w_{c}}) + \lambda_{pairwise}\cdot \sum_{a}\sum_{c_{i}, c_{j}\in a} L((\mathbf{x_{c_{i}}}-\mathbf{x_{c_{j}}})\mathbf{w_{s}}, (l_{c_{i}}-l_{c_{j}}))\\
&F_{c, 2}(\mathbf{w_{c}})=F_{c, 1}(w_{c}) +\\
& \lambda_{pairwise}\cdot \sum_{a}\sum_{c_{i}, c_{j}\in a} ((\mathbf{x_{c_{i}}}-\mathbf{x_{c_{j}}})\mathbf{w_{s}}- (l_{c_{i}}-l_{c_{j}}))^{2}
\end{split}
\end{equation}
}

%For some users, their comments are never picked up as editor-picks even they write hundreds of them. So 
We also hypothesize that comments from one user who never produces editor-picks may have similar "low" insightfulness. Thus our objective function becomes:

{\scriptsize
\begin{equation}
\begin{split}
&F_{c, 3}(\mathbf{w_{c}})=F_{c, 2}(\mathbf{w_{c}})+\lambda_{author}\cdot \sum_{u}\sum_{c_{i}, c_{j}\in C_{u}} (\mathbf{x_{c_{i}}}\mathbf{w_{c}}-\mathbf{x_{c_{j}}}\mathbf{w_{c}})^{2}\\
&=F_{c, 2}(w_{c})+\lambda_{author}\cdot \mathbf{w_{c}^{T}}\mathbf{X_{c}^{T}}\mathbf{L_{author}}\mathbf{X_{c}}\mathbf{w_{c}}
\end{split}
\end{equation}
}

Here $\mathbf{L_{author}}$ is another graph Laplacian defined based on whether two comments are written by the same user and that user's comments have never been selected as editor-picks.

\subsection{Connecting Sentences and Social Context}
Graph-based regularization learning techniques have been used in the space of web page classification \cite{Ji:2011:LST:2009916.2009928,Zhang:2006:LPM:1150402.1150510} and review quality prediction \cite{Lu:2010:ESC:1772690.1772761}. We utilize graph regularization to enforce similar sentences and social contexts that are relevant to topics having similar importance values.

{\scriptsize
\begin{equation}
\begin{split}
F_{s, c}(\mathbf{w_{s}}, \mathbf{w_{c}})= \lambda_{simi}\cdot \sum_{a}\sum_{s\in a, c\in a} R_{s, c} (\mathbf{x_{s}}\mathbf{w_{s}}-\mathbf{x_{c}}\mathbf{w_{c}})^{2}
\end{split}
\end{equation}
}

where $a$ is an article, $s$ is a sentence in the article, and $c$ is a comment in the article. $R_{s,c}$ indicates the similarity between the sentence and article.


\subsection{Full Objective Function}


So our final objective function should consist of the three main parts shown above:

{\scriptsize
\begin{equation}
\label{equa:full}
\begin{split}
F(\mathbf{w_{s}}, \mathbf{w_{c}})=F_{s, 2}(\mathbf{w_{s}})+F_{c, 3}(\mathbf{w_{c}})+F_{s, c}(\mathbf{w_{s}}, \mathbf{w_{c}})
\end{split}
\end{equation}
}


The \textbf{closed form solution} to the objective function in Equation~\ref{equa:full} is:

%\begin{equation}
%\end{equation}

\subsection{Features}
The features used to train the models for ranking sentences and comments are listed in Table~\ref{tab:features_sent} and Table~\ref{tab:features_comment}.


\begin{table}[ht]
\hspace{-5mm}
    {\fontsize{9}{10}\selectfont
    \setlength{\baselineskip}{0pt}
    
    \begin{tabular}{|l|l|}
    \hline
	\underline{\textbf{Basic Features}}& \underline{\textbf{Social Features}}\\ 
	- length &  - avg/sum frequency of  \\
	- absolute/relative position &  words mentioned in comment\\ 
	- first/first three sentences & - avg/sum frequency of  \\ 
	- avg/sum TF-IDF scores & dependency relations\\ 
	- \# NEs &   mentioned in comment\\ 
	- \# overlaps with headline & \\ \hline
	\end{tabular}
	}
    \caption{Features used for sentence ranking.} 
	\label{tab:features_sent}
\end{table}

\begin{table}[ht]
\hspace{-5mm}
    {\fontsize{9}{10}\selectfont
    \setlength{\baselineskip}{0pt}
    
    \begin{tabular}{|l|}
    \hline
	\underline{\textbf{Basic Features}}\\
	avg/sum of length \\
	user rating (positive-negative)\\
	num of sentences \\
	num/portion word types \\
	num/portion of capitalized words \\
	num/portion of NEs \\
	num of types of NEs \\
	avg/max/sum TF-IDF \\
	contain URL \\
	\hline	

	\underline{\textbf{Author Features}}\\
	num of comments posted by the author\\
	\hline
	
	\underline{\textbf{Readability Features}}\\ 
	Flesch–Kincaid Readability\\ 
	Gunning-Fog Readability\\
	\hline
	
	\underline{\textbf{Article Features}}\\ 
	TF/TF-IDF similarity with article\\
	TF/TF-IDF similarity with all the comments for the article\\
	JS/KL-divergence with article\\
	JS/KL-divergence with all the comments for the article\\
	\hline
	
	
	\underline{\textbf{Sentiment Features}}\\ 
	num/portion of positive/negative/neutral words (MPQA)\\
	num/portion of sentiment words\\
	\hline
	
	\underline{\textbf{Discourse Features}}\\
	num/portion of connectives\\
	num/portion of hedge words\\
	\hline
	\end{tabular}
	}
    \caption{Features used for comment ranking.} 
	\label{tab:features_comment}
\end{table}


==> setup.tex <==
\paragraph{Training the Joint Learning Model}
Gold-standard scores for sentences are computed against the human abstracts with ROUGE-2 scores. 
We reserved 20\% of the NYT2013 dataset for parameter tuning for joint learning model.


\paragraph{Gold-standard Timeline Summary}
The summary for each article will be under 100 words, and the number of comments 5.
We collect timeline summaries from Wikipedia webpages.

\paragraph{Preprocessing}
We get the parsing trees, dependency trees, and coreference resolution results of news articles and comments by Stanford CoreNLP~\cite{manning-etal:2014:ACLDemo}. We replace the mention of each entity with a uniform name with longest number of words (but no more than 5 words). 
The sentences in the articles are labeled with time information by using SUTime~\cite{chang12}. 

%\paragraph{Parameter Tuning}
%DUC2003 is also used for tuning parameters.
